A General Measure of Collision Hazard in Traffic

A collision hazard measure that has the essential characteristics to provide a measurement of safety that will be useful to AV developers, traffic infrastructure developers and managers, regulators and the public is introduced here. The Streetscope Collision Hazard Measure (SHM) overcomes the limitations of existing measures, and provides an independent leading indication of safety. * Trailing indicators, such as collision statistics, incur pain and loss on society, and are not an ethically acceptable approach. * Near-misses have been shown to be effective predictors of incidents. * Time-to-Collision (TTC) provides ambiguous indication of collision hazards, and requires assumptions about vehicle behavior. * Responsibility-Sensitive Safety (RSS), because of its reliance on rules for individual circumstances, will not scale up to handle the complexities of traffic. * Instantaneous Safety Metric (ISM) relies on probabilistic predictions of behaviors to categorize events (possible, imminent, critical), and does not provide a quantitative measure of the severity of the hazard. * Inertial Measurement Unit (IMU) acceleration data is not correlated with hazard or risk. * A new measure, based on the concept of near-misses, that incorporates both proximity (separation distance) and motion (relative speed) is introduced. * Near-miss data has been shown to be predictive of the likelihood and severity of incidents. The new measure presented here gathers movement data about vehicles continuously and a quantitative score reflecting the hazard encountered or created (from which the riskiness or safeness of the behavior of vehicles can be estimated) is computed nearly continuously.

==> convertDate.tex <==
%***************************************************************************
% \convertDate converts D:20080419103507+02'00' to 2008-04-19T10:35:07+02:00
%___________________________________________________________________________
\def\convertDate{%
    \getYear
}

{\catcode`\D=12
\gdef\getYear D:#1#2#3#4{\edef\xYear{#1#2#3#4}\getMonth}
}
\def\getMonth#1#2{\edef\xMonth{#1#2}\getDay}
\def\getDay#1#2{\edef\xDay{#1#2}\getHour}
\def\getHour#1#2{\edef\xHour{#1#2}\getMin}
\def\getMin#1#2{\edef\xMin{#1#2}\getSec}
\def\getSec#1#2{\edef\xSec{#1#2}\getTZh}
%\def\getTZh +#1#2{\edef\xTZh{#1#2}\getTZm}
\def\getTZh -#1#2{\edef\xTZh{#1#2}\getTZm}
\def\getTZm '#1#2'{%
    \edef\xTZm{#1#2}%
%    \edef\convDate{\xYear-\xMonth-\xDay T\xHour:\xMin:\xSec+\xTZh:\xTZm}%
    \edef\convDate{\xYear-\xMonth-\xDay T\xHour:\xMin:\xSec-\xTZh:\xTZm}%
}

\expandafter\convertDate\pdfcreationdate 
%___________________________________________________________________________

